AKE principles for deeply ramified fields

We study the model theory of deeply ramified fields of positive characteristic. Generalizing the perfect case treated in work by Jahnke and Kartas on the model theory of perfectoid fields, we obtain Ax-Kochen/Ershov principles for certain deeply ramified fields of positive characteristic and fixed degree of imperfection. Our results apply in particular to all deeply ramified henselian valued fields of rank 1.

==> preamble.tex <==
\usepackage[utf8]{inputenc}
%\usepackage[T1]{fontenc}
\usepackage[pdfusetitle]{hyperref}


% !TeX spellcheck = en_US


\usepackage{amsmath,amsthm,stackengine,scalerel}
\usepackage{amssymb}
\usepackage{mathrsfs}
\usepackage{mathtools}
\usepackage{tikz-cd}
\usepackage[shortlabels]{enumitem}
\usepackage[capitalise]{cleveref}
%\usepackage{dutchcal}
\usepackage{tikz}
\usepackage{todo}
\usepackage{fullpage}
\usepackage{parskip}

\RequirePackage[backend=bibtex,style=alphabetic,url=false]{biblatex}

%\usepackage{showkeys}


\usepackage{faktor}

\usepackage{csquotes}


\newtheoremstyle{mystyle}% name of the style to be used
{}% measure of space to leave above the theorem. E.g.: 3pt
{}% measure of space to leave below the theorem. E.g.: 3pt
{\normalfont}% name of font to use in the body of the theorem \bfseries \itshape \scshape \sfserief etc...\itfam
{}% measure of space to indent
{\bfseries}% name of head font
{}% punctuation between head and body
{0.5 em}% space after theorem head; " " = normal interword space
{\thmname{#1}\thmnumber{ #2}\normalfont\thmnote{ (#3)}\bfseries.}% Manually specify head

\newtheoremstyle{mystyle2}% name of the style to be used
{}% measure of space to leave above the theorem. E.g.: 3pt
{}% measure of space to leave below the theorem. E.g.: 3pt
{\itshape}% name of font to use in the body of the theorem \bfseries \itshape \scshape \sfserief etc...\itfam
{}% measure of space to indent
{\bfseries}% name of head font
{}% punctuation between head and body
{0.5 em}% space after theorem head; " " = normal interword space
{\thmname{#1}\thmnumber{ #2}\normalfont\thmnote{ (#3)}\bfseries.}% Manually specify head 

\newtheoremstyle{claimstyle}% name of the style to be used
{}% measure of space to leave above the theorem. E.g.: 3pt
{3pt}% measure of space to leave below the theorem. E.g.: 3pt
{}% name of font to use in the body of the theorem \bfseries \itshape \scshape \sfserief etc...\itfam
{}% measure of space to indent
{}% name of head font
{}% punctuation between head and body
{0.5 em}% space after theorem head; " " = normal interword space
{\underline{\thmname{#1}\thmnumber{ #2}\thmnote{ (#3)}:}}% Manually specify head 


\theoremstyle{mystyle2}
\newtheorem{thm}{Theorem}[section]
\newtheorem*{thm*}{Theorem}
\newtheorem{prop}[thm]{Proposition}
\crefname{prop}{Proposition}{Propositions}
\newtheorem{lem}[thm]{Lemma}
\newtheorem*{lem*}{Lemma}
\newtheorem{kor}[thm]{Corollary}

\theoremstyle{mystyle}
\newtheorem{defi}[thm]{Definition}
\newtheorem*{defi*}{Definition}
\crefname{defi}{Definition}{Definitions}
\newtheorem{examp}[thm]{Example}
\newtheorem*{examp*}{Example}
\newtheorem{rem}[thm]{Remark}
\newtheorem{obs}[thm]{Observation}
\newtheorem{fact}[thm]{Fact}
\newtheorem{prob}[thm]{Problem}
\newtheorem{Qu}[thm]{Question}

\theoremstyle{claimstyle}
\newtheorem{claim}{Claim}\counterwithin*{claim}{thm}

%%%%%%% personalised todo %%%%
\newcommand{\sylvytodo}[1]{\todo[linecolor=magenta,backgroundcolor=magenta]{\footnotesize #1}}
\newcommand{\margatodo}[1]{\todo[linecolor=red,backgroundcolor=red]{\footnotesize #1}}
\newcommand{\franzitodo}[1]{\todo[linecolor=blue,backgroundcolor=blue,textcolor=white]{\footnotesize #1}}
\newcommand{\margatodoinline}[1]{\todo[inline,backgroundcolor=red]{\footnotesize  #1}}
\newcommand{\sylvytodoinline}[1]{\todo[inline,backgroundcolor=magenta]{\footnotesize  #1}}
\newcommand{\franzitodoinline}[1]{\todo[inline,backgroundcolor=blue]{\footnotesize  #1}}


%%%%%%% math operators %%%%%%%
\DeclareMathOperator{\chara}{char}
\DeclareMathOperator{\id}{id}
\DeclareMathOperator{\res}{res}
\DeclareMathOperator{\resb}{\overline{res}}
\DeclareMathOperator{\rv}{rv}
\DeclareMathOperator{\ac}{ac}
\DeclareMathOperator{\acb}{\overline{ac}}
\newcommand{\vb}{\bar{v}}
\DeclareMathOperator{\discr}{discr}
\DeclareMathOperator{\Gal}{Gal}
\DeclareMathOperator{\ulim}{ulim}

\renewcommand{\vec}[1]{\underline{#1}}
\newcommand{\sort}[1]{\mathbf{#1}}
\newcommand{\struc}[1]{\mathcal{#1}}
\newcommand{\sostr}[2]{\sort{#1}(\struc{#2})}
\newcommand{\sostrn}[3]{\sort{#1}_{#2}(\struc{#3})}


%%%%%%% claim environment %%%%%%
\newcommand{\claimhead}[1]{\textbf{#1}}

\newenvironment{claim*}[1]{\par\noindent\underline{Claim:}\space#1}{}
\newenvironment{claimproof}[1]{\par\noindent\underline{Proof:}\space#1}{\hfill $\square_{\mathrm{Claim}}$\par}

%%%%%%% double bar %%%%%%
\renewcommand{\Bar}{\overline}
\stackMath
\def\stacktype{L}\setstackgap{L}{0pt}\def\useanchorwidth{T}
\def\barbar#1{\ThisStyle{\setbox0=\hbox{$\SavedStyle#1$}%
		\stackon{\SavedStyle#1}{\SavedStyle\hspace{.2\ht0}%
			\bar{\vphantom{#1}}\kern\dimexpr3.7\LMpt+1.7pt\relax\bar{\vphantom{#1}}}}%
}

\newcommand{\dbarv}{\barbar{v}}
\newcommand{\dbarw}{\barbar{w}}

\newcommand{\stdcplus}[2]{#1_{#2+}}
\newcommand{\stdcminu}[2]{#1_{#2-}}
\newcommand{\vtplus}{\stdcplus{v}{t}}
\newcommand{\vtminu}{\stdcminu{v}{t}}
\newcommand{\wsplus}{\stdcplus{w}{s}}
\newcommand{\wsminu}{\stdcminu{w}{s}}
\newcommand{\barvtminu}{\overline{\vtminu}}
\newcommand{\barwsminu}{\overline{\wsminu}}
\newcommand{\Ktplus}{\stdcplus{K}{t}}
\newcommand{\Ktminu}{\stdcminu{K}{t}}
\newcommand{\Lsplus}{\stdcplus{L}{s}}
\newcommand{\Lsminu}{\stdcminu{L}{s}}
\newcommand{\CoreField}[3]{\left(\stdcplus{#1}{#3},\overline{\stdcminu{#2}{#3}},\overline{#3}\right)}

\DeclareMathOperator{\Cf}{Cf}
\DeclareMathOperator{\Cfi}{Cf_i}
\DeclareMathOperator{\Tail}{Tail}

%%%%%%% notation %%%%%%%
\newcommand{\rdtame}{roughly divisible-tame}

%%%%%%% math symbols shortcuts %%%%%%
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\F}{\mathbb{F}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\R}{\mathbb{R}}

\let\polishL\L%polish L because I am evil
\newcommand{\Losthm}{\polishL{}o\'s's theorem}%Los I'm lazy

\DeclareMathOperator{\Th}{Th}

\DeclareMathOperator{\Quot}{Quot}
\newcommand{\asclose}[1]{{#1}^{\text{AS}}}

\newcommand{\sep}{^\mathrm{sep}}
\newcommand{\alg}{^\mathrm{alg}}

%\DeclareMathSymbol{\Gamma}{\mathord}{operators}{"00}
\newcommand{\U}{\mathcal{U}}
\newcommand{\V}{\mathcal{V}}

\newcommand{\C}{\mathcal{C}}

\newcommand{\Lang}{\mathcal{L}}
\newcommand{\Lring}{\L_{\mathrm{ring}}}
\newcommand{\Loag}{\L_{\mathrm{oag}}}
\newcommand{\Lhyp}{\L_{\mathrm{hyp}}}
\newcommand{\Lval}{\L_{\mathrm{val}}}
\newcommand{\Lthree}{\L_{\Gamma k}}
\newcommand{\LRVzero}{\L_{\RV_0}}
\newcommand{\LRV}{\L_\RV}

\newcommand{\LPas}{\L_{\mathrm{Pas}}}
\newcommand{\Lac}{\L_{\ac}}

\newcommand{\Henzz}{\mathsf\barwU{Hen}_{00}}
\newcommand{\Henz}[1]{\mathsf{Hen}_{0 #1}}
\newcommand{\Henzzac}{\Henzz^{\mathrm{ac}}}
\newcommand{\Henzpac}{\Henz{p}^{ac}}

\renewcommand{\O}{\mathcal{O}}
\newcommand{\m}{\mathfrak{m}}
\newcommand{\RV}{\mathrm{RV}}

\newcommand{\barv}{\overline{v}}
\newcommand{\barvp}{\overline{v_p}}
\newcommand{\barvt}{\overline{v_t}}
\newcommand{\barvpU}{\overline{v_p{}^\U}}
\newcommand{\barvU}{\overline{v^\U}}
\newcommand{\barvUp}{\overline{v^\U{}_p}}
\newcommand{\barw}{\overline{w}}
\newcommand{\barwp}{\overline{w_p}}
\newcommand{\barwpU}{\overline{w_p{}^\U}}
\newcommand{\barwU}{\overline{w^\U}}
\newcommand{\barwUp}{\overline{w^\U{}_p}}
\newcommand{\baru}{\overline{u}}

\newcommand{\x}{^\times}

\newcommand{\powerfield}[1]{\left(\!\left(#1\right)\!\right)}

%%%%%%%%%%%%hyphenation%%%%%%%%%%%%%%%
\hyphenation{hen-se-lian}



\newcommand\SA[1]{{\color{blue}{\bf SA}:#1}}
